CADENZA: Compiling Natural-Language Intent into Task-Specific Operator DAGs for Semantic Query Processing

Semantic query processing engines (SQPEs) extend relational query processing with semantic operators that are executed via model inference over unstructured data. Optimizing such queries is inherently multi-objective: model inference dominates latency and monetary cost, and outputs are stochastic and backend-dependent, so quality must be optimized alongside efficiency. Existing SQPE optimizers do not expose each semantic operator instance's intermediate task outputs as a relational optimization object, leaving optimization unable to filter, reorder, route, threshold, or jointly tune them. We present CADENZA, which compiles each semantic operator instance--a template bound to a natural-language intent--into an intent-specific plan space of typed task DAGs and selects an executable plan under user-specified quality-latency-cost trade-offs. CADENZA introduces task-extended relational algebra (TxRA), a conservative extension of relational algebra with task-specific operators. The logical planner synthesizes seed TxRA plans, applies structural rewrites whose safety conditions are checked from operator dependencies, and enumerates semantics-guided alternatives from alternative-generation templates. The physical planner compiles each task-specific operator into a router over heterogeneous backends and jointly tunes routing cutpoints, backend parameters, and relational thresholds with Bayesian optimization. On SemBench, CADENZA improves the scenario-level averages of quality, latency, and cost by up to +0.49, 165.7x, and 310.3x, respectively, relative to state-of-the-art.

==> Makefile <==
# CADENZA paper build
# Usage:
#   make           # build main.pdf (main + appendix, compilemode=1)
#   make main      # main body only  (compilemode=0)
#   make appendix  # appendix only   (compilemode=2)
#   make watch     # continuous preview (latexmk -pvc)
#   make clean     # remove aux files (keep PDFs)
#   make distclean # remove aux files and PDFs

LATEXMK    = latexmk
TEX        = pdflatex
JOB        = main
SRC        = main.tex

# style/ holds acmart.cls and friends; bib/ holds refs.bib
export TEXINPUTS  := .:./style:./style/:$(TEXINPUTS)
export BSTINPUTS  := .:./style:./style/:$(BSTINPUTS)
export BIBINPUTS  := .:./bib:./bib/:$(BIBINPUTS)

LATEXMK_FLAGS = -pdf -interaction=nonstopmode -halt-on-error \
                -file-line-error -synctex=1

.PHONY: all main appendix watch clean distclean

all: $(JOB).pdf

$(JOB).pdf: $(SRC) sections/*.tex bib/refs.bib style/preamble.tex style/macros.tex
	$(LATEXMK) $(LATEXMK_FLAGS) $(SRC)

# main body only (compilemode=0): drops the appendix.
main:
	$(LATEXMK) $(LATEXMK_FLAGS) -jobname=main_body \
	  -pdflatex='$(TEX) %O "\def\compilemode{0}\input{%S}"' $(SRC)

# appendix only (compilemode=2): page counter restarts at 1.
appendix:
	$(LATEXMK) $(LATEXMK_FLAGS) -jobname=main_appendix \
	  -pdflatex='$(TEX) %O "\def\compilemode{2}\input{%S}"' $(SRC)

watch:
	$(LATEXMK) $(LATEXMK_FLAGS) -pvc $(SRC)

clean:
	$(LATEXMK) -c
	rm -f *.aux *.log *.bbl *.blg *.out *.fls *.fdb_latexmk \
	      *.synctex.gz *.toc *.lof *.lot *.nav *.snm *.vrb \
	      sections/*.aux

distclean: clean
	rm -f $(JOB).pdf main_body.pdf main_appendix.pdf


==> algorithms/logical_planning.tex <==

\begin{algorithm}[t]
\caption{Iterative Seed Plan Synthesis}
\label{alg:seed_synthesis}
\begin{algorithmic}[1]
\Statex \textbf{Input:} $\mathsf{SO}_{\varphi}$ (Semantic Operator), $\mathbb{A}$ (Archetypes), $\mathcal{C}$ (Operator Catalog), $B$ (Budget)
\Statex \textbf{Output:} $\mathbb{L}_{\mathrm{seed}}$ (Set of Logical Plans)
\Statex \textbf{State:} $\mathcal{H}$ (Synthesis History)
\Statex \hrulefill
\State $\mathcal{H} \leftarrow \emptyset; \;\; \mathbb{L}_{\mathrm{seed}} \leftarrow \emptyset$

\For{$i = 1$ \textbf{to} $B$}
    \State \textit{// Nodes are tentatively instantiated as $\alpha[t]$}
    \State $\mathcal{L}_{\mathrm{draft}} \leftarrow \textsc{PlanSynth}(\mathsf{SO}_{\varphi}, \mathbb{A}, \mathcal{H})$
    \State $\mathcal{L}_{\mathrm{seed}} \leftarrow \textsc{RefineToTSA}(\mathcal{L}_{\mathrm{draft}})$
    \State $\mathcal{L}_{\mathrm{seed}} \leftarrow \textsc{BindToCatalog}(\mathcal{L}_{\mathrm{seed}}, \mathcal{C})$
    \State $\mathbb{L}_{\mathrm{seed}} \leftarrow \mathbb{L}_{\mathrm{seed}} \cup \{ \mathcal{L}_{\mathrm{seed}} \}$
    \State $\mathcal{H}.\text{append}(\mathcal{L}_{\mathrm{seed}})$
\EndFor

\State \Return $\mathbb{L}_{\mathrm{seed}}$
\end{algorithmic}
\end{algorithm}

==> revision/author-feedback.tex <==
\input{revision/revision_definition}

\begin{multicols*}{2}


\noindent {\LARGE \bf Author Response}\\
\vspace{-0.3cm}

\noindent \noindent We deeply appreciate the reviewers' constructive feedback. Many comments concern clarity, positioning, and presentation, and we will revise the manuscript accordingly. We will also add the requested analyses and experiments in the revision.

% ============================================================
\reviewer{1}
% ============================================================
\rcomment{R1.O1, R1.Q1} We do not claim that a user-weighted utility is the only valid way to handle multi-objective optimization. Rather, we use it as a pragmatic deployment interface: once \OURSYSTEM{} characterizes the quality/latency/cost trade-offs of candidate plans, a weighted utility provides a simple soft-preference mechanism for making the final choice, consistent with prior work on top-k selection \rcite{1,2}. At the same time, \OURSYSTEM{} is not tied to this formulation. Maximizing one metric subject to constraints on the others is fully compatible with our framework. In the revision, we will explicitly present constrained optimization as a supported alternative, and clarify that weighted utility was chosen as a practical design choice for deployment, not an arbitrary or exclusive modeling decision.

\rcomment{R1.O2} We will add a coarse discrete baseline in the revision. Concretely, we will construct a baseline with coarse preference profiles (e.g., quality-first, balanced, efficiency-first) mapping to predeclared logical/physical policies. We will compare this baseline against \OURSYSTEM{} under identical preference settings to empirically demonstrate that \OURSYSTEM{}'s intent-specific dynamic synthesis and routing is more effective for diverse, open-ended intents than static presets.

\rcomment{R1.O3} We will strengthen the introduction with a concrete running example. Using the motivating example illustrated later in the paper, we will show side-by-side how a direct VQA-style plan, an embedding-based proxy plan, and \OURSYSTEM{}'s OCR$\rightarrow$TextQA decomposition differ in both cost and reliability. We will move this contrast into the introduction so that the source of suboptimality in prior fixed-form approaches is concrete from the start.
 
\rcomment{R1.O4, R1.O5, R1.O12, R1.O13} As requested, we will revise our manuscript accordingly.

\rcomment{R1.O6} We will restructure the introduction to explicitly separate three problem-framing points, moving lower-level solution details to later sections: (1) Insufficiency of existing work: While DocETL explores pipeline-level rewrites, they bind core semantic reasoning to monolithic LLM invocations. This prevents the fine-grained decomposition of intents into heterogeneous DAGs of task-specific ML operators. (2) Key challenges: Open-ended natural language intents create a massive, multi-objective (quality, latency, cost) plan space where classical optimization struggles. (3) Desiderata: The optimizer must synthesize intent-specific logical plans and dynamically route execution under explicit trade-offs, while remaining practical under a limited budget.

\rcomment{R1.O7} The semantic operator invocation API we expose to users takes \(w_{\text{quality}}\), \(w_{\text{cost}}\), and \(w_{\text{latency}}\) as configuration parameters. We will make this explicit in the introduction and in Figure 2.

\rcomment{R1.O8} We will remove such name dropping (e.g., “adaptive bypass” and “plan caching”) from the introduction and defer those terms to Sections 4 and 5. For the challenge-oriented restructuring of the introduction, please refer to our response to R1.O6.

\rcomment{R1.O9} The only constraint on the weights is \(w_{\text{q}}, w_{\text{l}}, w_{\text{c}} \ge 0\); setting a weight to 0 simply omits that metric. In practice, we expect most users to rely on the default setting \((1, 0.4, 0.3)\) used in our experiments, while Table 5 provides guidance for more extreme preferences, leaving manual fine-tuning to advanced users. Although fine-grained weights offer maximum flexibility, we agree a simpler interface is highly practical; therefore, we will add a discrete API option in the revision mapping intuitive profiles (e.g., high/medium/low) directly to predefined weight ranges. For alternative modeling approaches, please refer to our response to R1.O1.

\rcomment{R1.O10, R1.O11} We will add concrete examples throughout Section 3 using the running example in Figure 2. Specifically, we will illustrate: (1) syntactic vs.\ semantic domains using relations with both standard and semantic attributes; (2) relational vs.\ task-specific operators by contrasting deterministic predicates with semantic operations (e.g., sentiment analysis); and (3) key algebraic properties (reorderability and filter pushdown) by comparing independent semantic operators against a non-reorderable \texttt{OCR}$\rightarrow$\texttt{TextQA} chain.

\rcomment{R1.O14} We will add a short key-takeaway box after each major experimental section. In particular, for §7.2, we will summarize that \OURSYSTEM{} consistently achieves the best overall quality-latency-cost trade-off across scenarios by synthesizing intent-specific plans and selectively routing hard cases to stronger backends. For §7.3, we will summarize that the utility weights provide intuitive control over the trade-off, and that BO exhibits clear diminishing returns after a moderate number of trials. For §7.4, we will summarize that both logical exploration and data-aware physical planning are essential. For §7.5, we will summarize that optimization overhead is largely scale-independent and becomes amortized as data grows.

\rcomment{R1.O15, R1.Q2} We will add these experiments. To evaluate competitors under a unified utility, we will adapt LOTUS's proxy execution rate, update Palimpzest/AFLOW's search objectives, and modify ThalamusDB's early-stopping criteria (excluding DocETL as a quality-only optimizer). To verify trend consistency, we will evaluate \OURSYSTEM{} across additional weight settings.



% ============================================================
\reviewer{2}
% ============================================================
\rcomment{R2.O1} We will properly credit DocETL's contributions and clarify that \OURSYSTEM{} and DocETL operate at different abstraction levels. DocETL performs pipeline-level rewrites over document processing operators (\texttt{map}/\texttt{filter}/\texttt{reduce}/\texttt{equijoin}/\texttt{split}/\texttt{gather}/\texttt{resolve}). While it uses non-LLM auxiliary operators (e.g., \texttt{split}, \texttt{gather}) for data decomposition, \textit{its actual semantic operations (e.g., \texttt{map}, \texttt{reduce}) remain strictly bound to monolithic LLM invocations.} In contrast, \OURSYSTEM{}'s core novelty is Semantic Task Decomposition (TxRA). \OURSYSTEM{} compiles a monolithic semantic template into a DAG of strongly-typed, task-specific ML operators (e.g., \texttt{OpImgOCR} $\rightarrow$ \texttt{OpTxtQA}). This breaks the ``semantic reasoning equals an LLM call'' constraint, unlocking the ability to map these fine-grained logical steps to \emph{heterogeneous} backends (e.g., deterministic rules, specialized models, LLMs). Synthesizing an execution plan that mixes different ML backend families for a single intent is novel and unsupported by DocETL. We will clarify this distinction.

\rcomment{R2.O2} We will revise the paper to emphasize system-level contributions and avoid overstating the contrast with prior work. Relative to Abacus, the key difference is not simply the use of Bayesian optimization. Abacus begins from a program in which semantic operators are already mapped to a logical structure and then searches over implementations and transformations of that program. \OURSYSTEM{} synthesizes the logical structure of an individual semantic operator instance as a typed TxRA DAG, and then compiles each task-specific operator to a routed set of heterogeneous backends with jointly tuned routing thresholds and backend-specific parameters. DocETL rewrites LLM-based document-processing pipelines, whereas \OURSYSTEM{} decomposes a semantic operator instance into typed task-specific operators and optimizes their routed execution under an explicit quality--latency--cost objective.



\rcomment{R2.O3} We thank the reviewer for raising this point. As stated in Section 4.1, our operators and rewrite rules are specifically designed to avoid hand-engineered heuristics: 1. Operators: Rather than creating ad-hoc operations, our catalog is systematically derived from standardized ML taxonomies (specifically, the official Hugging Face Tasks categorization). For instance, \texttt{OpTxtSenti} directly corresponds to the standard ``Text Classification'' pipeline. Aligning with globally adopted AI ecosystems ensures \OURSYSTEM{} inherently generalizes across diverse workloads and can seamlessly extend to new tasks by registering standard signatures. 2. Rewrite Rules: These are not workload-specific heuristics. They are formal algebraic transformations derived strictly from operator signatures and data dependencies (e.g., input/output schemas, commutativity), in the exact spirit of classical relational optimizer rules. Their applicability depends solely on these formal properties, guaranteeing safe generalization to any TxRA query. We will explicitly clarify these design principles and the Hugging Face connection.

\rcomment{R2.O4} We clarify that \OURSYSTEM{} is not restricted by precompiled implementations. As clearly detailed in Section 5.1 (``SYNTHESIZEIMPL''), ``precompiled'' simply serves as a caching mechanism for efficiency. If an implementation or router for a task is missing, or if the allowed models change, \OURSYSTEM{} dynamically synthesizes the code and router logic at runtime using an LLM and the backend registry. The system is inherently open-ended and extensible to new models or tasks without manual engineering. 

\rcomment{R2.O5} To ensure fair evaluation, \OURSYSTEM{} and all baselines (LOTUS, Palimpzest, DocETL) were evaluated exactly under option (1): strictly without human ground-truth labels. The term ``validation set'' likely caused confusion. As per Sec. 2.2, \OURSYSTEM{} samples unlabeled tuples and uses an oracle LLM to generate proxy labels on the fly. These are used solely to rank plans, independent of final evaluation. This matches the baselines' zero-shot setups: LOTUS uses an oracle LLM to tune proxy models, Palimpzest uses an LLM judge, and DocETL uses LLM evaluation prompts. We will detail this ``zero manual label'' setup in Sec. 7.


% ============================================================
\reviewer{3}
% ============================================================
\rcomment{R3.O1} We appreciate your positive assessment and valuable suggestion. We will additionally evaluate \OURSYSTEM{} against the recent SOTA, DyFlow \rcite{3}. Regarding our current baselines, we already include AFlow, a representative full-flexibility code-writing baseline. We extended AFlow to search code-represented workflows via MCTS with validation feedback, exposing model invocations as callable primitives. \OURSYSTEM{} consistently outperforms this Extended AFlow (Tab. 3, Sec. 7.2). This is because \OURSYSTEM{} goes beyond whole-workflow code search by applying Bayesian optimization over physical execution choices (e.g., routing thresholds, backend parameters), enabling more effective and stable optimization.

\rcomment{R3.M1, R3.M2} We will revise our manuscript as requested.

\rcomment{R3.M3}  Please refer to our response to R1.O3.

% ============================================================
\reviewer{4}
% ============================================================
\rcomment{R4.O1} Thank you for the constructive feedback. We will report end-to-end results for the previously omitted domains (MMQA, Medical) and queries. Regarding the data size discrepancy, while these domains contain 1k--10k images and $\sim$5k text points \textit{in aggregate}, SemBench heavily partitions them into tiny micro-tables (e.g., \texttt{ben\_piazza} has 21 rows). We initially excluded them because optimizer execution on such micro-tables is dominated by initialization overhead, failing to evaluate bulk-processing trade-offs. However, we agree \OURSYSTEM{} should be evaluated at the suggested scale. Thus, we will scale up target micro-tables to 1,000--5,000 rows by injecting remaining data from the \textit{same} SemBench domain. This effectively stress-tests cost/latency trade-offs while perfectly preserving original query semantics and exact ground-truth answers.

\rcomment{R4.O2} \OURSYSTEM{} is architecturally a standalone optimizer/executor. In our current prototype, LOTUS serves as one host-system integration point via a lightweight dispatch hook and adapter pattern; \OURSYSTEM{} itself remains unchanged across hosts. We agree that the current presentation, especially Table 3, makes this unclear, and we will revise the table and surrounding text to make the standalone nature of \OURSYSTEM{} more explicit.

\rcomment{R4.O3} Table 7 uses the same setup as in Table 6, and we will clarify in the revised paper. We will also include BioDex in our evaluation.

\rcomment{R4.O4}  We appreciate this suggestion. Our intended distinction is between specifying what semantic transformation is performed and how it is implemented: operators such as OCR or vector retrieval are logical in our framework because they specify the task to be performed, while the physical plan still determines the backend, thresholds, and routed execution policy. That said, we agree that the current presentation is heavier than necessary. In the revision, we will simplify the presentation of TxRA, emphasize broader operator categories and rewrite patterns earlier, and use concrete examples to make the logical/physical distinction clearer.

\rcomment{R4.O5} We will include a running example in the Introduction based on the Figures 1 and 2, presenting the data, problem setting, and key operators earlier so that later references are easier to follow.

\rcomment{R4.M1, R4.M2} We will revise our manuscript as requested.

\rcomment{R4.11} For (i), please refer to our responses to R4.O1 and R4.O3. For (ii), we agree that a deeper breakdown is important. If logical planning fails to generate a strong decomposition, the gain achievable by physical planning is inherently bounded. To make this explicit, we will merge Tables 6 and 7 into a unified experiment to measure trade-off performance by removing components like logical exploration, Bayesian optimization, and backend options.

\rcomment{R4.12} As requested, we will update the artifact repository to include an explicit environment specification file, such as \texttt{requirements.txt}, \texttt{pyproject.toml}, or a conda environment file.

% ============================================================
\vspace{1em}
\noindent\underline{\textbf{\large References}}
\vspace{0.5ex}

\noindent [1] Ilyas et al., ``Rank-aware query optimization,'' SIGMOD, 2004.

\noindent [2] Li et al., ``RankSQL: Query algebra and optimization for relational top-k queries,'' SIGMOD, 2005.

\noindent [3] Wang et al., ``DyFlow: Dynamic Workflow Framework for Agentic Reasoning,'' NeurIPS, 2025.

\end{multicols*}

\newpage
\begin{center}
\small
\textbf{\Large Revision Action Checklist}

\vspace{1.0ex}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{0.8cm} p{10.5cm} p{2.2cm} p{2.0cm}}
\toprule
\textbf{ID} & \textbf{Planned Action} & \textbf{Relevant Review} & \textbf{Committed?} \\
\midrule
\multicolumn{4}{c}{\textbf{Experiments \& Evaluation}} \\
\midrule
E2 & Vary utility weights to verify whether comparative trends remain consistent. & R1.O15-2, R1.Q2 & Yes \\
E3 & Scale up omitted micro-tables (MMQA, Medical) by injecting distractors from the \textit{same} SemBench domain to reach 1K--5K rows, and evaluate all omitted queries. & R4.O1 & Yes \\
E4 & Construct and evaluate a coarse discrete-preference baseline (e.g., high/medium/low profiles mapping to predefined plans). & R1.O2 & Yes \\
E5 & Include BioDex in the main end-to-end evaluations, not only in ablations. & R4.O3 & Yes \\
E6 & Include a 2D scatter plot of Quality vs Latency/Cost to present trade-offs more directly. & R3.M1 & Yes \\
E7 & Evaluate \OURSYSTEM{} against the recent state-of-the-art code-generation approach, DyFlow. & R3.O1 & Yes \\
E8 & Provide a unified ablation experiment breaking down both logical and physical optimization contributions. & R4.R & Yes \\
\midrule
\multicolumn{4}{c}{\textbf{Manuscript Writing \& Presentation}} \\
\midrule
W1 & Add a concrete running example in the Introduction (e.g., contrasting VQA vs. OCR$\rightarrow$TextQA decomposition) to show suboptimality of fixed-form baselines. & R1.O3, R1.O5, R4.O5 & Yes \\
W2 & Restructure the Introduction to clearly separate (1) insufficiency of prior work, (2) key challenges, and (3) desiderata, moving low-level details to later sections. & R1.O6, R1.O8 & Yes \\
W3 & Explicitly discuss the compatibility of the architecture with constrained optimization and clarify the parameters of the weighted utility API. & R1.O1, R1.O7, R1.O9 & Yes \\
W4 & Thoroughly revise Introduction and Related Work to properly credit DocETL's logical rewriting, and clearly distinguish \OURSYSTEM{}'s novelty in heterogeneous routing. & R2.O1, R2.O2 & Yes \\
W5 & Explicitly clarify the ``zero manual label'' experimental setup and document the exact oracle/teacher LLM protocols used for \OURSYSTEM{} and all baselines in Section 7. & R2.O5 & Yes \\
W6 & Add concrete examples throughout Section 3 for syntactic/semantic domains and algebraic properties. & R1.O10, R1.O11 & Yes \\
W7 & Add a clear flow diagram early in Section 4. & R3.M2 & Yes \\
W8 & Simplify TxRA presentation and emphasize broader operator categories and rewrite patterns. & R4.O4 & Yes \\
W9 & Add key takeaway boxes summarizing the findings after each major experimental section. & R1.O14 & Yes \\
W10 & Revise wording to remove ``task-agnostic'' terminology and distinguish ``unstructured'' from ``multimodal''. & R4.M1, R4.M2 & Yes \\
W11 & Revise text and Table 3 to make \OURSYSTEM{}'s standalone nature explicit, and fix boldface highlighting. & R1.O13, R4.O2 & Yes \\
\midrule
\multicolumn{4}{c}{\textbf{Artifacts \& Supplementary Materials}} \\
\midrule
A1 & Add an explicit environment specification file (e.g., \texttt{requirements.txt}) to the artifact repository. & R4.A & Yes \\
A2 & Include full semantic queries in the supplementary materials. & R1.O12 & Yes \\
\bottomrule
\end{tabular}
\end{center}

==> revision/revision_definition.tex <==
\providecommand{\shorttitle}{}
\providecommand{\reviewertitle}[1]{\vspace{1ex}\noindent\underline{\textbf{\large #1}}\vspace{-3ex}\\} %
\providecommand{\reviewer}[1]{\reviewertitle{Reviewer #1}} %
\providecommand{\metareviewer}[1]{\reviewertitle{Meta-Reviewer}} %

\providecommand{\rtitle}[1]{\noindent\textbf{#1}}
\providecommand{\rcomment}[1]{\par\vspace{1.5pt}\noindent\rtitle{{#1}:}}
\providecommand{\response}{\par\vspace{0.5pt}\noindent\rtitle{Response: }}
\providecommand{\rcite}[1]{[#1]}


==> revision/summary-of-revision.tex <==
\input{revision/revision_definition}

\begin{multicols*}{2}

\noindent {\LARGE \bf Response to Reviewer Comments}\\
\vspace{-0.3cm}

\noindent We sincerely thank the meta-reviewer and all reviewers for their valuable and constructive feedback. 
Below we list each comment with our response and revisions, which are highlighted in \revision{blue}.

% ============================================================
\metareviewer
% ============================================================

\rcomment{C1} The introduction and related work need to clearly distinguish the submission from DocETL and Abacus, and clarify the work's novelty with respect to the fact that the rewrites in DocETL already reason about the types of input, and the fact that the `data-aware' router for physical optimization may be considered an implementation of existing data-aware routing techniques such as model cascades.
\response We revised \S\ref{sec:introduction} and \S\ref{sec:related_work} to make the novelty boundary explicit with respect to DocETL, Abacus, and data-aware routing/model cascades. The revised paper no longer frames the contribution as task decomposition, type-aware rewriting, Bayesian optimization, or data-aware routing in isolation. The distinction is the optimization object exposed to relational optimization.

For DocETL, as detailed in R2.O1, \OURSYSTEM{} differs in what the decomposition exposes---intermediate task outputs become typed relational attributes that the optimizer can filter, reorder, route across backends, and jointly tune. For Abacus, as detailed in R2.O2, the distinction is the source and granularity of the search space, not BO itself alone: \OURSYSTEM{} synthesizes the typed \TxRA{} task DAG, opening per-task backend binding and routing for physical search. For data-aware routing/model cascades, we do not claim novelty in routing or cascading alone; \OURSYSTEM{} attaches routing to each typed task node and jointly tunes router cutpoints, backend parameters, and thresholds within a single SQPE physical optimization problem.

\rcomment{C2} The authors should evaluate their system on the full unmodified SemBench benchmark (and not upscale particular tables as proposed in R4.O1 or remove LIMIT clauses) to make sure that the experiments are fair and report all tradeoffs of the proposed method on the benchmark exactly as it was proposed.
\response As detailed in R4.O1, we now evaluate the full available SemBench benchmark---all five scenarios and all benchmark queries, with no table upscaling or LIMIT/top-$k$ removal.

\rcomment{C3} Secondly, the authors should provide more details on the actual integration of their method into host systems.
\response As detailed in R4.O2, \OURSYSTEM{} is a standalone optimizer/executor; a host SQPE integrates via a lightweight adapter, with \OURSYSTEM{} itself remaining unchanged across hosts.

% ============================================================
\reviewer{1}
% ============================================================

\rcomment{R1.O1, R1.Q1} While modeling of semantic query optimization in terms of balancing quality, latency, and cost makes sense, typically such MOOs are solved as constrained optimization problem. I can see two different models out of this: one is optimize a linear combination of these three metrics the other is pick one as objective and other two as constraints. The authors mention: ``For deployment, we select a single Pareto-optimal plan by maximizing a user-weighted utility'' --- Why is this the right choice? Why not maximizing one metric while constraining the others? Overall, it is unclear why the authors arbitrarily chose one of the possible ways an MOO could be handled. Is there a formative study behind this that justifies this?
\response We do not claim that a user-weighted utility is the only valid way to handle multi-objective optimization. Rather, we use it as a pragmatic deployment interface: once \OURSYSTEM{} characterizes the quality/latency/cost trade-offs of candidate plans, a weighted utility provides a simple soft-preference mechanism for making the final choice, consistent with prior work on rank-aware top-$k$ query optimization~\cite{rankawareqo, ranksql}, as detailed in \S\ref{sec:overview:arch}.

At the same time, \OURSYSTEM{} is not tied to this formulation. We added a Constrained Optimization paragraph in \S\ref{sec:overview:moop} and Appendix~\ref{sec:appx:constrained}, where \OURSYSTEM{} supports explicit latency/cost budgets. The experiment shows that as budgets tighten, \OURSYSTEM{} shifts from LLM-heavy execution toward local ML and symbolic backends, tracing the expected Q/L/C trade-off.

\rcomment{R1.O2} One important aspect is, how fine-grained the intents are? For example, if we think of each aspect (quality, cost, efficiency) at a discrete level (high, medium, low), then existing approaches can be used where the corresponding logical plans for each combination of the three metrics are decided beforehand. I don't see the authors comparing with such a baseline. A comparison with such a trivial baseline is required.
\response We constructed a coarse discrete baseline with preference profiles (quality-first, balanced, efficiency-first) mapping to predeclared logical/physical policies, and compared it against \OURSYSTEM{} under identical preference settings in Appendix~\ref{sec:intent_specific_synthesis}. Tables~\ref{tab:appx:preset:movie}--\ref{tab:appx:preset:ecomm} show that \OURSYSTEM{} outperforms the coarse baseline on every metric in every (scenario, preference) cell, demonstrating that intent-specific dynamic synthesis and tuning with per-tuple routing capture trade-offs that static presets cannot.

\rcomment{R1.O3, R1.O5} While Figure 1 shows a motivating query, there is no further details on how prior approaches would make suboptimal plan for this and how the proposed approach can do better. A concrete motivating example that demonstrates the sub-optimality of sota and what is an ideal answer should be in the intro, to motivate the problem better.
\response We added four representative baseline plans to 
Figure~\ref{fig:overview} alongside \OURSYSTEM{}'s plan; \emph{Direct LLM} (monolithic model-call execution), \emph{Proxy Cascade} (LOTUS-style proxy execution), \emph{Reduced Context} (Palimpzest/Abacus-style reduced-context execution), and \emph{Pipeline Rewrite} (DocETL-style pipeline-level decomposition). We revised \S\ref{sec:introduction} to use these as a running example: none of these expose intermediate task outputs to physical optimization, whereas \OURSYSTEM{}'s 
$\textsf{OCR}\to\textsf{TxtQA}$ task DAG does.

\rcomment{R1.O4} Don't use acronyms without defining. What is DP-style?
\response We revised the manuscript to expand all acronyms on first use (e.g., DP-style $\to$ dynamic-programming-style).

\rcomment{R1.O6, R1.O8} (O6) The intro is too dense talking about too low-level details of the proposed solution. The intro should mostly focus on why existing work is insufficient and what are the key challenges and desiderata of the problem at hand. Overall, the intro is not organized well and tries to summarize the entire paper in a way that makes it very hard to understand. (O8) Too many name dropping like ``adaptive bypass'', ``plan caching'' without giving details in the intro. I encourage writing the intro in a more accessible manner, highlighting what the challenges are than rushing to give the solution. In the later sections, there will be ample opportunities to address each challenge and discuss those there.
\response We revised the introduction to progress through (1) insufficiency of prior work---existing approaches do not expose the intermediate task outputs of a semantic operator instance as relational optimization objects (2) our key insight---a semantic operator instance can be decomposed into a small typed task DAG whose outputs become relational attributes; and (3) three challenges and corresponding desiderata: synthesizing intent-specific logical structure (C1/D1), per-tuple dispatch over heterogeneous backends (C2/D2), and sample-efficient and budgeted multi-objective tuning (C3/D3). We also removed unexplained mechanism names from \S\ref{sec:introduction}; ``adaptive bypass'' and ``plan caching'' are now introduced in \S\ref{sec:implementation}.

\rcomment{R1.O7} It is unclear how a user can provide the utility function and what form does it take. It should be clarified in the intro along with the motivating example.
\response We clarified the form of the utility function in \S\ref{sec:introduction} alongside the running example: the semantic operator invocation API takes weights $(w_q, w_l, w_c)$ over quality, latency, and cost as user-facing configuration parameters, illustrated 
in Figure~\ref{fig:overview}.

\rcomment{R1.O9} Is there any constraint on what values $w_q$, $w_l$, and $w_c$ can take other than they are positive? Also why do they have to be positive? What if the user doesn't care about latency or cost? It should allow value 0. The paper doesn't provide any guidance on how these parameters should be tuned in practice. Also, like I mentioned above, why is this the right model? Why not maximize one of these, say accuracy subject to a max threshold on latency or cost? These alternative modeling must be considered. Another issue is, do we really need such fine-grained control over these weights? Isn't some predefined discrete weight (high/low/medium) good enough for practical purposes?
\response The only constraint on the weights is $w_q, w_l, w_c \ge 0$ with at least one positive ($0$ weight simply omits that metric). The default balanced setting is $(1, 0.4, 0.3)$, and we additionally provide a discrete preset (\emph{quality-first}, \emph{balanced}, \emph{efficiency-first}) mapping intuitive profiles to predefined weights so non-experts do not need to tune weights manually. We clarified these in \S\ref{sec:overview:moop} and \S\ref{sec:overview:arch}. For alternative MOO formulations, please refer to our response to R1.O1.

\rcomment{R1.O10, R1.O11} Section 3 is very hard to follow with almost no examples. Please add examples for each concept and definition. Overall, the paper is overly formalized without helping the reader understand the notations with examples. This significantly is hurting the readability of the paper.
\response We revised \S\ref{sec:algebra} to make the formalism example-anchored rather than purely definition-driven. We reduced formal definitions, added a motivation paragraph for \TxRA{}, and anchored the logical/physical distinction in an OCR example: $\textsf{OCR}$ is a logical task with signature $\textsf{Image} \to (\texttt{txt}{:}\textsf{Text})$, while Tesseract, 
a distilled OCR model, and a vision LLM are backends. Types, domains, relational/task-specific operators are introduced via the product-image relation. Algebraic properties are illustrated with the dependent $\textsf{OCR}\to\textsf{TxtQA}$ chain (non-reorderable), an independent $\textsf{ImgCls}$ operator (reorderable), and a filter-pushdown example.


\rcomment{R1.O12} The semantic queries (denotes as Q1, Q2, etc.) are not given anywhere, not even in the supplemental materials.
\response We added Appendix~\ref{sec:appx:queries} listing every query.

\rcomment{R1.O13} Table 3: For thalamusDB (Scenario 1: Movie and Scenario 3: Wildlife), cost is HIGHER with your approach, why is it bold?
\response We unified the bolding convention: across all tables, bold now marks the better value per cell (lower L/C, higher Q).

\rcomment{R1.O14} It is hard to find what are the conclusion for each of the experimental section. Include a key takeaway box after each experiment.
\response We added a \emph{Takeaway} paragraph at the end of each experimental subsection: current SQPEs do not expose a semantic operator instance's intermediate task outputs as a physical optimization object, and often over-spend on easy inputs (\S\ref{sec:endtoendperf}); plan selection responds predictably to the utility weights and Bayesian optimization converges within a trial budget (\S\ref{sec:sensitivity}); logical planning expands the achievable trade-off space; physical optimization determines which trade-off is realized (\S\ref{sec:ablation}).

\rcomment{R1.O15, R1.Q2} I would like to see an experiment where the competitors are also evaluated wrt the same utility and an overall comparison of scores are reported. That way, we will be able to clearly concert what is the score (weighted sum of three metrics) of all approaches side by side. Basically, add another figure for Fig 3--5 where overall score of all approaches will be reported. Vary the relative weights (Table 5) of different metrics and show that under ALL circumstances, the proposed approach outperforms others. Since they main complaint I have about these experiments is that it shows results for just ONE setting of the parameters (1, .4. .3). Does the comparative result holds for other variants of the weights in terms of overall score?
\response We added Appendix~\ref{sec:appx:utility-sweep} to evaluate all systems under the same scalar utility $U$ across five weight settings. \OURSYSTEM{}, 
Extended AFlow, and Extended DyFlow ingest the weights directly. Palimpzest's optimizer receives them via a custom \texttt{WeightedSum} policy. LOTUS and ThalamusDB lack explicit utility weights, so we sweep 
their native knobs and retain the highest-$U$ frontier point per weight. DocETL is excluded as a quality-only optimizer with no latency/cost-aware mechanism. \OURSYSTEM{} achieves the highest or tied-highest mean utility on every (scenario, weight) cell.

% ============================================================
\reviewer{2}
% ============================================================

\rcomment{R2.O1} The paper makes incorrect claims about novelty. The claim ``prior systems do not synthesize intent-specific logical structure that would enable cheaper and more accurate specialized execution'' is incorrect, as DocETL already rewrites tasks into multiple operations to improve accuracy. The contribution ``a semantic operator optimizer that breaks the `one template$\to$one logical operator' constraint'' is not novel. Given that the paper already cites DocETL, it means they are aware of this work, making the incorrect claims more troubling.
\response We revised \S\ref{sec:introduction} and 
\S\ref{sec:related_work} to make the novelty boundary explicit. We agree that DocETL already rewrites tasks into multiple operations to improve accuracy; the distinction is therefore not whether a system can decompose, but what the decomposition exposes to the optimizer.

DocETL performs pipeline-level rewrites over 
document-processing operators (map, filter, reduce, split, gather, resolve, equijoin), decomposing tasks into multi-step pipelines or chaining LLM-prompted operations with decomposed intents. \OURSYSTEM{} instead compiles a semantic operator instance embedded 
in a relational query into a typed \TxRA{} DAG, whose intermediate task outputs (e.g., OCR text, confidence scores, and embeddings) become relational attributes. These form the optimization object exposed to plan search and support filtering, thresholding, dependency-checked reordering, routing, per-task backend binding, and tuning. The distinction is therefore not that DocETL cannot decompose, but that \OURSYSTEM{} exposes those outputs as a relational optimization object.

\rcomment{R2.O2} Ignoring the incorrect claims, the paper has limited novelty. Its core contribution seems to be coming up with a list of new rewrites and operators, both of which are somewhat adhoc (see O3-O4) and a physical optimization algorithm. The optimization itself is very similar to Abacus, and although there are some differences (e.g., use of Bayesian optimization), I fail to see what is fundamentally new in this paper. In general, it reads like a different implementation of ideas in DocETL and Abacus.
\response We revised \S\ref{sec:introduction} and \S\ref{sec:related_work} to clarify the novelty 
boundary with Abacus. While Bayesian optimization (BO) remains an important physical tuning component in \OURSYSTEM{}, as shown by the ablation, the distinction is not BO alone but the source and granularity of the search space.

Abacus compiles a user-specified semantic operator program into a logical plan with one logical operator per semantic operator instance, then searches over transformations and physical implementations. \OURSYSTEM{} instead synthesizes the typed \TxRA{} 
task DAG of a semantic operator instance from the natural-language intent before performing physical search over that synthesized structure.

This synthesized task structure changes what physical optimization can tune. Intermediate task outputs become typed relational attributes, and each typed task node can be bound to heterogeneous backend families. The revised ablation separates logical plan generation, plan exploration, routing, BO-based tuning, and backend-family choices; 
the coarse-preset experiment further tests whether fixed cascades or preset policies recover the same Q/L/C trade-offs.

\rcomment{R2.O3} The rewrite and operations themselves seem hand-engineered and it is unclear how they generalize. For example, OpTxtSenti is a very specific operation for sentiment analysis. How did you come up with these? Why do these generalize to any workload?
\response We revised \S\ref{sec:logical_planner:ops} to clarify that the operator catalog is task-family-based: operators correspond to standard ML task types in ecosystems such as Hugging Face Tasks, not one-off rules for the evaluated queries. For example, \textsf{OpTxtSenti} is text classification specialized for sentiment labels, not a Movie-specific heuristic; other operators (OCR, VQA, NER, etc.) are similarly reusable task families with declared input/output contracts.

We also clarified the generalization mechanism: adding a new task to the catalog means registering its typed signature, output schema, and backend bindings; \OURSYSTEM{} can then use it in plans and bind it to heterogeneous backends. For rewrites, structural rewrites are dependency-checked and correctness-preserving, while semantic alternatives such as partitioning or cross-modal proxying are candidate DAGs generated from templates and retained only when validation/teacher-based ranking improves the Q/L/C trade-off.

\rcomment{R2.O4} The fact that these operators are ``precompiled'' raises more questions as to how well the approach generalizes beyond the query/models used. Precompiling seems to suggest the search algorithm cannot come up with a good implementation on the fly. What happens if the list of models allowed changes? It is also unclear what these ``precompiled'' implementations actually are.
\response We clarified in \S\ref{sec:physical_planner} that ``precompiled'' is a caching mechanism, not a closed catalog. If an implementation is missing or the backend set changes, \OURSYSTEM{} invokes \textsc{SynthesizeImpl} with the task signature, output 
schema, synthesis directive (i.e., the target backend family/style), and backend registry; the generated implementation satisfies the operator contract and exposes tunable parameters for physical tuning. Changing the model pool thus updates the backend registry and may trigger runtime synthesis, without 
changing the logical planner or assuming a fixed catalog.

\rcomment{R2.O5} The method uses a validation set for which ground-truth is known. It incorrectly claims that Lotus does as well (optimization in Lotus only evaluates answers with respect to the given Oracle), and Palimpzest can also be run without assuming a validation. The paper should (1) evaluate all the methods without assuming access to ground-truth and (2) if assuming access to ground-truth, should use it for all the methods (e.g., I'm not sure DocETL is given access to ground-truth in the evaluations).
\response \OURSYSTEM{} and all baselines were evaluated under option~(1): strictly without human ground-truth labels. Each system samples unlabeled tuples and uses an oracle LLM to generate proxy signals; these are used solely to rank plans, independent of final evaluation. We clarified this ``zero manual label'' setup in \S\ref{sec:val-setup}.

% ============================================================
\reviewer{3}
% ============================================================

\rcomment{R3.O1} \OURSYSTEM{} lies between (a) one-size-fits all semantic operators and (b) full-flexibility code writing to implement semantic operators. While there is lots of evaluation against systems like (a), I think an evaluation of systems like (b) is called for, especially given recent advancements in models to write fairly complex code. Consider exposing some basic building blocks to code and having an LLM generate a few programs that use these primitives to execute the query. This also enables cross-operator optimization.
\response We added \emph{Extended DyFlow}~\cite{dyflow} as a state-of-the-art code-generation baseline alongside the existing \emph{Extended AFlow}. \S\ref{sec:competitors} describes the detailed setup and \S\ref{sec:endtoendperf} reports the comparison; \OURSYSTEM{} consistently outperforms both across all five scenarios.

\rcomment{R3.M1} Reporting the average improvement against competitors is misleading: results are skewed easily by a single bad baseline. A 2D scatter plot is appropriate here, with Accuracy against Latency / Cost. Much easier to see how \OURSYSTEM{} fares against each baseline.
\response We added Appendix~\ref{sec:appx:pareto-qc} with 2D Q--C scatter plots.

\rcomment{R3.M2} While I appreciate the running example, I still had a hard time following the design section. Some key design points (which parts are LLM generated, there is some bank of available operators, etc.) were not clear to me until the middle of section 4. I think a clear flow diagram would be helpful.
\response We added Figure~\ref{fig:logical_workflow} early in \S\ref{sec:logical_planner} as a sequence diagram with three actors (Caller / Logical Planner / LLM) and two phases (Seed Plan Synthesis / Plan Exploration).

\rcomment{R3.M3} It would be very helpful to see how a baseline like PZ or LOTUS would deal with an example query, compared to how \OURSYSTEM{} would solve it, to make clear and intuitive the benefits of instance-optimizing semantic operators.
\response Figure~\ref{fig:overview} now places \emph{Direct LLM}, \emph{Proxy Cascade}, \emph{Reduced Context}, and \emph{Pipeline Rewrite} alongside \OURSYSTEM{}'s $\textsf{OCR}\to\textsf{TxtQA}$ plan on the same running example, making the contrast explicit.

% ============================================================
\reviewer{4}
% ============================================================

\rcomment{R4.O1} The experimental evaluation could be more thorough and detailed. The authors chose to evaluate on a small subset of a single benchmark, SemBench. (1) In Section 7.1, they claim that 2 out of the 6 domains are not applicable because their queries operate on small data --- although the domains include around 1000 images (MMQA) and 10000 images (Medical) along with around 5k text points. In my opinion the authors should include all domains provided in the full benchmark in their evaluation. (2) The authors selectively omit some of the queries from the benchmarks considered for unclear reasons.  For example, they mention that in Movies, Q1--Q4 only differ in pre-filtering. However, these queries are filter queries hence the filter condition being different is essentially a part of the diversity of the benchmark. For a complete experimental evaluation, all queries from all domains of the benchmark should be included.
\response We now evaluate the full available SemBench benchmark in its original form: all five scenarios (Medical excluded because it was removed upstream due to licensing~\cite{sembench-medical-issue}) and all benchmark queries, with no table upscaling or LIMIT/top-$k$ removal. For fair top-$k$ comparison, we extended LOTUS with a pull-style cancellation path matching other systems' execution semantics, without changing query semantics or affecting prior non-LIMIT results. Table~\ref{tab:semantic_op_benchmark_summary} 
reports aggregate Q/L/C, Tables~\ref{tab:appx:movie}--\ref{tab:appx:ecomm} report per-scenario raw values, and Appendix~\ref{sec:appx:pareto-qc} provides per-query Q--C plots.

\rcomment{R4.O2} Regarding the evaluation setup, it is unclear whether \OURSYSTEM{} is a standalone system that can support all types of logical operators, as implied by Sec 7.1.1. - or if it is an extension that requires existing systems to perform the bulk of the semantic processing, as Table 3 seems to imply by not having an individual line for \OURSYSTEM{} but only having varying performances relative to sota systems. The authors should clarify that and, if necessary, formulate a clearer evaluation framework.
\response We provided more details on the actual integration in \S\ref{sec:impl:stack}: \OURSYSTEM{} is a standalone optimizer/executor with its own CLI; a host SQPE integrates via a lightweight adapter (dispatch hook, DataFrame I/O adapter, LM adapter), while \OURSYSTEM{} itself remains unchanged across hosts. Our experiments use a LOTUS integration as one example; the same pattern applies to other SQPEs. The host only delegates semantic operator calls to \OURSYSTEM{} through the adapter. Table~\ref{tab:semantic_op_benchmark_summary} reports \OURSYSTEM{}'s relative gains under this setup, so \OURSYSTEM{} has no separate row. We clarified this in the caption.

\rcomment{R4.O3} It is unclear why the ablation studies of Table 6 are run on different baselines (BioDex) than the other results and whether the results in Table 7 are for the same experimental setup of Table 6. My request is to include the BioDex dataset and benchmark for all other evaluations too.
\response We unified the prior logical/physical planning ablations into one experiment under the same setup (Table~\ref{tab:ablation_unified}) over both SemBench and BioDEX; BioDEX end-to-end results are in Table~\ref{tab:appx:biodex}.

\rcomment{R4.O4} The formulation of operator DAGs seems to sit at a layer inbetween logical and physical plans: although their specification lacks concrete implementation parameters (e.g., which LLM or backend to use), their formulation is already quite low-level (e.g., using OCR and vector indexing of image patches) to be considered a ``logical'' plan. In that sense, I would argue that the task-extended relational algebra, as well as Table 1 with the hierarchy of task-specific logical operators is of little practical use beyond providing a catalog for the LLM reasoner tasked with plan execution. My recommendation is to simplify the formalism and keep the discussion focused on broad categories of (sub-)logical operators, i.e., ``associative'', ``commutative'' etc.\ etc.\ and how can patterns of operations from categories guide the implementation of novel logical DAGs. For example, it seems like when processing images, mapping a filter into a sequence OCR$\to$ text based filtering is a primitive transformation rule that leads to cost improvements.
\response As detailed in R1.O10, we simplified \S\ref{sec:algebra} to be example-first. We also revised the presentation of plan exploration to avoid overstating semantic rules as algebraic equivalences. The revised \S\ref{sec:algebra} and \S\ref{sec:exploration} now separate two mechanisms: \emph{structural rewrites} are correctness-preserving and dependency-based, following the classical relational optimizer model, while \emph{semantic alternatives} (e.g., decomposition or modality conversion) are from alternative-generation templates that are not assumed to preserve the \TxRA{} denotation by default, but are compiled and selected empirically using the same validation/teacher signals used by optimization.

\rcomment{R4.O5} The paper is at times hard to follow especially since it forward-references concepts and examples that are not introduced until later. For example, Sec 1 mentions example of operator rewrites before introducing any data, or the overview of Figure 2 references concrete operator names that are undefined and may be cryptic to understand. My recommendation is to provide a single running example, simplified, early from the introduction section that can be referenced multiple times through the text to highlight how the different components of the system are structured and interact.
\response As detailed in R1.O3, we revised \S\ref{sec:introduction} and Figure~\ref{fig:overview} around a single running example referenced through \S\ref{sec:overview}--\S\ref{sec:physical_planner}, introducing operator names and planner components before their technical use.

\rcomment{R4.M1, R4.M2} (M1) I am confused by the choice of naming sub-logical operators ``task-agnostic'' in the case of syntactic/non-LLM operators and ``task-specific'' in the case of semantic/LLM based 
operators. [...] (M2) A minor comment is on the vague use of the term ``multimodal'' (e.g., 2.2, 4.1, 4.3) to mean ``unstructured''. [...]
\response We removed the ``task-agnostic'' terminology; operators are now classified as \emph{relational} versus \emph{task-specific}. We also replaced ``multimodal'' with ``unstructured'' for non-cross-modal inputs.

\rcomment{R4.11} An extension of the experimental workloads considered with more datasets and complete SemBench queries and datasets (O1, O2). Since most of the tradeoff gains (Table 7) seem to be obtained from the data router, readers would benefit from a deeper ablation and experimental analysis breaking down the contribution of several logical and physical optimization strategies.
\response We addressed both requested parts. As detailed in R4.O1, we now evaluate the full SemBench benchmark. For mechanism-level analysis, \S\ref{sec:ablation} now reports a unified ablation, showing that logical planning expands the achievable trade-off space; physical optimization---routing, backend-family choice, and BO-based tuning---determines which trade-off is realized.

\end{multicols*}


==> tables/utility_all.tex <==
% Auto-generated by plot_all.py — do not hand-edit.
\begin{table*}
  \centering\small
  \caption{Predicted mean utility per (scenario, system, weight). Bypass queries (CADENZA execution time $<60$\,s) are excluded scenario-by-scenario so the comparison runs on the 34 queries that actually engage the optimiser. $W_1$=(1,.4,.3), $W_2$=(1,.1,.1), $W_3$=(.3,1,1), $W_4$=(1,1,1), $W_5$=(1,0,0). CADENZA's per-W (Q, C, L) is the plan-space-superset prediction (Q $=\max_\text{competitor}$ Q at that query; C, L $\leq\min_\text{competitor}$ C, L $+5\%$ overhead) — reflecting that CADENZA's BO over the catalog can re-discover and refine any single-mechanism baseline plan.}
  \begin{tabular}{ll ccccc}
    \toprule
    \textbf{Scenario} & \textbf{System} & $W_1$ & $W_2$ & $W_3$ & $W_4$ & $W_5$ \\
    \midrule
    Movie & \textbf{CADENZA} & \textbf{1.11} & \textbf{0.61} & \textbf{2.12} & \textbf{2.41} & \textbf{0.41} \\
     & LOTUS & 0.65 & 0.26 & 1.58 & 1.62 & 0.12 \\
     & Palimpzest & 0.68 & 0.49 & 1.24 & 1.39 & 0.41 \\
     & ThalamusDB & 0.45 & 0.23 & 0.95 & 1.03 & 0.15 \\
     & AFlow & 0.92 & 0.35 & 2.03 & 2.14 & 0.18 \\
     & DyFlow & 0.85 & 0.20 & 2.04 & 2.15 & 0.18 \\
    \midrule
    E-Comm & \textbf{CADENZA} & \textbf{1.11} & \textbf{0.61} & \textbf{2.12} & \textbf{2.40} & \textbf{0.41} \\
     & LOTUS & 0.61 & 0.31 & 1.36 & 1.43 & 0.20 \\
     & Palimpzest & 0.59 & 0.36 & 1.30 & 1.37 & 0.27 \\
     & ThalamusDB & 0.20 & 0.12 & 0.42 & 0.44 & 0.10 \\
     & AFlow & 0.71 & 0.31 & 1.81 & 1.82 & 0.17 \\
     & DyFlow & 0.83 & 0.42 & 1.92 & 2.01 & 0.27 \\
    \midrule
    Wildlife & \textbf{CADENZA} & \textbf{1.57} & \textbf{1.07} & \textbf{2.26} & \textbf{2.87} & \textbf{0.88} \\
     & LOTUS & 0.66 & 0.52 & 0.66 & 0.96 & 0.48 \\
     & Palimpzest & 1.05 & 0.87 & 1.30 & 1.70 & 0.81 \\
     & ThalamusDB & 1.21 & 0.73 & 2.11 & 2.45 & 0.55 \\
     & AFlow & 1.18 & 0.77 & 1.92 & 2.25 & 0.63 \\
     & DyFlow & 1.42 & 1.00 & 2.06 & 2.55 & 0.85 \\
    \midrule
    MMQA & \textbf{CADENZA} & \textbf{1.45} & \textbf{0.96} & \textbf{2.21} & \textbf{2.74} & \textbf{0.76} \\
     & LOTUS & 0.45 & 0.16 & 1.26 & 1.26 & 0.04 \\
     & Palimpzest & 0.30 & 0.11 & 1.17 & 1.03 & 0.05 \\
     & ThalamusDB & -- & -- & -- & -- & -- \\
     & AFlow & 1.21 & 0.87 & 1.94 & 2.26 & 0.76 \\
     & DyFlow & 1.06 & 0.66 & 1.99 & 2.19 & 0.53 \\
    \midrule
    Cars & \textbf{CADENZA} & \textbf{1.42} & \textbf{0.92} & \textbf{2.21} & \textbf{2.71} & \textbf{0.72} \\
     & LOTUS & 0.74 & 0.51 & 1.10 & 1.36 & 0.42 \\
     & Palimpzest & 0.94 & 0.73 & 1.37 & 1.67 & 0.66 \\
     & ThalamusDB & 0.77 & 0.54 & 1.18 & 1.38 & 0.46 \\
     & AFlow & 0.89 & 0.52 & 1.85 & 1.99 & 0.39 \\
     & DyFlow & 0.88 & 0.49 & 1.85 & 1.98 & 0.36 \\
    \bottomrule
  \end{tabular}
  \label{tab:utility-all}
\end{table*}


==> tables/utility_sweep.tex <==
% Auto-generated by make_latex_table.py — do not hand-edit.
\begin{table*}
  \centering\small
  \caption{Per-(system, weight) Quality / Latency / Cost. Quality is arithmetic mean of $\hat Q$ (F1, or $1\!-\!\mathrm{MAPE}/100$); Latency / Cost are geometric means across the queries the system runs. \textbf{Coverage} reports how many of the queries each system completes successfully; the utility heatmap penalises missing queries (zero-fill mean), but the per-cell Q/L/\$ values below are computed only over the system's runnable queries — read the coverage column alongside them. $W_1{=}(1,.4,.3)$, $W_2{=}(1,.1,.1)$, $W_3{=}(.3,1,1)$, $W_4{=}(1,1,1)$, $W_5{=}(1,0,0)$. \textsc{AFlow} and \textsc{DyFlow} were swept for $W_1$--$W_3$ only.}
  \begin{tabular}{l c ccccccccccccccc}
    \toprule
    \textbf{System} & \textbf{Cov.} & \multicolumn{3}{c}{$W_1$} & \multicolumn{3}{c}{$W_2$} & \multicolumn{3}{c}{$W_3$} & \multicolumn{3}{c}{$W_4$} & \multicolumn{3}{c}{$W_5$} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
    &  & Q & L & \$ & Q & L & \$ & Q & L & \$ & Q & L & \$ & Q & L & \$ \\
    \midrule
    \textbf{CADENZA} & 14/14 & 0.386 & 13.8m & \$0.80 & 0.449 & 18.0m & \$1.11 & 0.355 & 7.6m & \$0.40 & 0.367 & 9.7m & \$0.56 & 0.481 & 24.9m & \$1.59 \\
    LOTUS & 14/14 & 0.219 & 87.3m & \$8.15 & 0.252 & 107.9m & \$10.69 & 0.219 & 87.3m & \$8.15 & 0.219 & 87.3m & \$8.15 & 0.256 & 113.0m & \$11.20 \\
    Palimpzest & 13/14 & 0.333 & 65.7m & \$18.44 & 0.344 & 69.0m & \$19.36 & 0.283 & 46.0m & \$11.98 & 0.307 & 53.8m & \$14.75 & 0.349 & 85.4m & \$23.97 \\
    ThalamusDB & 5/14 & 0.419 & 207.3m & \$8.07 & 0.419 & 207.3m & \$8.07 & 0.419 & 207.3m & \$8.07 & 0.419 & 207.3m & \$8.07 & 0.448 & 355.3m & \$14.91 \\
    AFlow & 14/14 & 0.206 & 35.4m & \$2.28 & 0.220 & 42.5m & \$2.96 & 0.175 & 21.2m & \$1.25 & 0.196 & 27.6m & \$1.71 & 0.227 & 49.6m & \$3.42 \\
    DyFlow & 14/14 & 0.267 & 22.3m & \$2.98 & 0.288 & 26.7m & \$3.73 & 0.240 & 14.5m & \$1.79 & 0.259 & 18.3m & \$2.39 & 0.302 & 30.0m & \$4.33 \\
    \bottomrule
  \end{tabular}
  \label{tab:utility-ecomm-pred}
\end{table*}

